Improved Algorithm on Online Clustering of Bandits

We generalize the setting of online clustering of bandits by allowing non-uniform distribution over user frequencies. A more efficient algorithm is proposed with simple set structures to represent clusters. We prove a regret bound for the new algorithm which is free of the minimal frequency over users. The experiments on both synthetic and real datasets consistently show the advantage of the new algorithm over existing methods.

==> Improved Algorithm on Online Clustering of Bandits/Algorithm.tex <==
\section{Algorithm}
\label{sec:algorithms}

\begin{algorithm}[t]
\caption{\sclub}
\label{alg:sclub}
\begin{algorithmic}[1]
\STATE \textbf{Input}: exploration parameter $\alpha_{\theta}, \alpha_p > 0$, and $\beta > 0$;
\STATE \label{algoline: user initialization} Initialize information for each user $i \in [n_u]$ by $S_i = \bI_{d \times d}, b_i = \mathbf{0}_{d \times 1}, T_i = 0$;
\STATE \label{algoline: cluster initialization} Initialize the set of cluster indexes by $J = \{1\}$ and initialize the single cluster by $S^1 = \bI_{d \times d}, b^1 = \mathbf{0}_{d \times 1}, T^1 = 0, C^1 = [n_u], j(i) = 1,\forall i$;
\FOR{\label{algoline: for s} $s =1, 2, \dots$}
\STATE \label{algoline: mark users unchecked} Mark every user unchecked for each cluster;
\STATE \label{algoline: set pivot} For each cluster $j$, compute $\tilde{\bT}^j = \bT^j$, %$\tilde{\bp}^j = \bT^j / (|\bC^j| T)$, 
and $\tilde{\btheta}^j = (\bS^j)^{-1} \bb^j$;
\FOR{\label{algoline: for t} $t = 1, \ldots, 2^s$}
\STATE \label{algoline: compute total time step tau} Compute the total time step $\tau = 2^s - 2 + t$;
\STATE \label{algoline: receive user and item set Dt} Receive a user $\bi_{\tau}$ and an item set $\bD_{\tau} \subset \RR^d$;
\STATE \label{algoline: get cluster index and its associated information} Get the cluster index $\bj = \bj(\bi_\tau)$ and its associated information $(\bS^{\bj}, \bb^{\bj}, \bT^{\bj})$;
% \IF{\label{algoline: if Sj is invertible} $\bS^{\bj}$ is invertible}
\STATE \label{algoline: recommend item to the user with largest U} Recommend item $\bx_{\tau} = \argmax_{x \in \bD_{\tau}} \bU(x)$ where
\begin{align*}
\bU(x) = (\bb^{\bj})^\top (\bS^{\bj})^{-1} x + \beta \norm{x}_{(\bS^{\bj})^{-1}}
\end{align*}
to user $\bi_{\tau}$ and receive feedback $\by_{\tau}$
% \ELSE
% \STATE \label{algoline: randomly select item from Dt} Randomly select item $\bx_{\tau}$ from $\bD_{\tau}$ and receive feedback $\by_{\tau}$;
% \ENDIF
\STATE Run \textbf{Update}
\STATE Run \textbf{Split}
\STATE Mark user $\bi_\tau$ has been checked;
\STATE Run \textbf{Merge}
\ENDFOR{~~$t$}
\ENDFOR{~~$s$}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Update}
\label{alg:update}
\begin{algorithmic}
\STATE Update the information for user $\bi_{\tau}$ and cluster $\bj$
\begin{align*}
&\bS_{\bi_{\tau}} = \bS_{\bi_\tau} + \bx_{\tau} \bx_{\tau}^{\top},  \quad \bb_{\bi_\tau} = \bb_{\bi_\tau} + \by_{\tau} \bx_{\tau}, \\
&\bT_{\bi_\tau} = \bT_{\bi_\tau} + 1, \quad \hat{\bp}_{\bi_{\tau}} = \bT_{\bi_\tau} / \tau, \\
&\hat{\btheta}_{\bi_\tau} = \bS_{\bi_{\tau}}^{-1} \bb_{\bi_\tau},\\
&\bS^{\bj} = \bS^{\bj} + \bx_{\tau} \bx_{\tau}^{\top},  \quad \bb^{\bj} = \bb^{\bj} + \by_{\tau} \bx_{\tau}, \\
&\bT^{\bj} = \bT^{\bj} + 1, \quad \hat{\bp}_{i'} = \bT_{i'} / \tau, ~~\forall i' \in \bC^{\bj},\\
&\hat{\btheta}^{\bj} = (\bS^{\bj})^{-1} \bb^{\bj}\,.
\end{align*}		
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Split}
\label{alg:split}
\begin{algorithmic}
\STATE $F(T) = \sqrt{\frac{1 + \ln(1 + T)}{1 + T}}$;
\IF{ \label{algoline: check split} $\norm{\hat{\btheta}_{\bi_\tau} - \tilde{\btheta}^{\bj}} > \alpha_{\theta} \left(F(\bT_{\bi_\tau}) + F(\tilde{\bT}^{\bj})\right)$ or there exists user $i' \in \bC^{\bj}$ with $\abs{\hat{\bp}_{\bi_\tau} - \hat{\bp}_{i'}} > 2 \alpha_p F(\tau)$}
\STATE /\ /\ Split user $\bi_\tau$ from cluster $\bj$ and form a new cluster $j' (= \max J + 1)$ of user $\bi_\tau$
\begin{align*}
&\bS^{\bj} = \bS^{\bj} - \bS_{\bi_\tau} + \bI, \quad \bb^{\bj} = \bb^{\bj} - \bb_{\bi_\tau}, \\
&\bT^{\bj} = \bT^{\bj} - \bT_{\bi_{\tau}}, \quad \bC^{\bj} = \bC^{\bj} - \{\bi_\tau\};\\
&\bS^{j'} = \bS_{\bi_{\tau}}, \quad \bb^{j'} = \bb_{\bi_\tau}, \quad \bT^{j'} = \bT_{\bi_{\tau}}, \quad \bC^{j'} = \{\bi_\tau\}
\end{align*}
\ENDIF
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Merge}
\label{alg:merge}
\begin{algorithmic}
\FOR{ any two checked clusters $j_1 < j_2$ satisfying
\begin{align*}
\norm{\hat{\btheta}^{j_1} - \hat{\btheta}^{j_2}} < \frac{\alpha_{\theta}}{2} \left(F(\bT^{j_1}) + F(\bT^{j_2})\right)
\end{align*}
and
\begin{align*}
\abs{\hat{\bp}^{j_1} - \hat{\bp}^{j_2}} < \alpha_p F(\tau) 
\end{align*}
}
\STATE /\ /\ Merge them: add information of cluster $j_2$ to cluster $j_1$ and remove cluster $j_2$
\begin{align*}
&\bS^{j_1} = \bS^{j_1} + \bS^{j_2} - \bI\,, \quad \bb^{j_1} = \bb^{j_1} + \bb^{j_2}\,, \\
&\bT^{j_1} = \bT^{j_1} + \bT^{j_2}\,, \quad \bC^{j_1} = \bC^{j_1} \bigcup \bC^{j_2}\,; \\
\vspace{-0.2in}
&j(i) = j_1 ~~\forall i \in \bC^{j_2} \text{ and delete cluster } j_2
\end{align*}
\ENDFOR{}
\end{algorithmic}
\end{algorithm}

\ifsup
\begin{figure}[thb!]
\centering
\begin{tikzpicture}[scale=0.7,font=\small]

\node at (0,0) {(a) The Split Operation};
\draw[->, very thick] (-0.7,-1.5) -- (0.7,-1.5);
\node at (-4, -1) {$1$};
\node at (-3.2, -1) {$2$};
\node at (-2.4, -1) {$3$};
\node at (-4, -2) {$4$};
\node at (-3.2, -2) {$5$};
\node at (-2.4, -2) {$6$};
\draw (-3.2,-1.5) ellipse (1.4cm and 1cm);
\draw[dashed] (-2.4,-1) circle (0.3cm);

\node at (2.4, -1) {$1$};
\node at (3.2, -1) {$2$};
% \node at (3, -1) {$3$};
\node at (2.4, -2) {$4$};
\node at (3.2, -2) {$5$};
\node at (4, -2) {$6$};
\draw (3.2,-1.5) ellipse (1.4cm and 1cm);
\node at (5, -1) {$3$};
\draw (5,-1) circle (0.3cm);

\node at (0,-3.5) {(b) The Merge Operation};
\draw[->, very thick] (-0.7,-5) -- (0.7,-5);
\node at (-4.5, -4.5) {$1$};
\node at (-3.7, -4.5) {$2$};
\node at (-1.9, -4.5) {$3$};
\node at (-4.5, -5.5) {$4$};
\node at (-2.7, -5.5) {$5$};
\node at (-1.9, -5.5) {$6$};
\draw (-4.1,-5) ellipse (0.8cm and 1cm);
\draw (-2.3,-5) ellipse (0.8cm and 1cm);

\node at (2.4, -4.5) {$1$};
\node at (3.2, -4.5) {$2$};
\node at (4, -4.5) {$3$};
\node at (2.4, -5.5) {$4$};
\node at (3.2, -5.5) {$5$};
\node at (4, -5.5) {$6$};
\draw (3.2,-5) ellipse (1.4cm and 1cm);
\end{tikzpicture}
\caption{The illustrations of the split and merge operations on sets.}
\label{fig:split merge}
\end{figure}
\fi

In this section, we introduce our algorithm of ``set-based clustering of bandits (\sclub)'' to deal with the online clustering of bandit problem. Recall that the related previous work \cite{gentile2014online,li2016collaborative} adopted connected components in graphs to represent clusters and the learning process only split clusters. In contrast, our algorithm uses sets to represent clusters and allow both split and merge operations on sets in the learning process. 
\ifsup
\cref{fig:split merge} provides an illustration of the split and merge operations on sets. The learner will split a user out of the current set if it finds inconsistency between the user and the cluster (\cref{fig:split merge}a); the learner will merge two existing clusters if they are close enough (\cref{fig:split merge}b). The meanings of inconsistency and similarity will be explained later. 
\fi
The pseudocode is provided in \cref{alg:sclub}.

In the algorithm, we store a profile of $(\bS_i, \bb_i, \bT_i)$ for each user $i$, where $\bT_i$ is the number of times that the user $i$ has appeared, $\bS_i$ is the Gramian matrix and $\bb_i$ is the moment vector of regressand by regressors. For example, if $(x_1, y_1), \ldots, (x_n, y_n)$ are pairs of items and corresponding rewards collected for user $i$ before time $t$, then 
\begin{align*}
    T_i = n\,, \quad S_i = \sum_{k=1}^{n} x_k x_k^\top\,, \quad b_i = \sum_{k=1}^{n} x_k y_k\,.
\end{align*}
The user profiles are initialized in the beginning of the algorithm (line \ref{algoline: user initialization}), and the clustering is initialized to be a single set with index $1$ containing all users (line \ref{algoline: cluster initialization}). We store a profile of $(\bS^j, \bb^j, \bT^j, \bC^j)$ for each cluster $j$, where $\bC^j$ is the set of all user indexes in this cluster and
\begin{align*}
\bS^j = \bI+\sum_{i \in \bC^j} (\bS_i - \bI), \quad \bb^j = \sum_{i \in \bC^j} \bb_i, \quad \bT^j = \sum_{i \in \bC^j} \bT_i
\end{align*}
are the aggregate information in the cluster $j$. As a convention, we use subscript $\bS_i, \bb_i, \bT_i$ to denote the information related to a user $i$ and use superscript $\bS^j, \bb^j, \bT^j$ to denote the information related to a cluster $j$.

The learning agent proceeds in phases (line \ref{algoline: for s}), where the $s$-th phase contains $2^s$ rounds (line \ref{algoline: for t}). Each phase has an accuracy level such that the learner could put accurate clusters aside and focus on exploring inaccurate clusters. In the beginning of each phase, mark every user to be unchecked (line \ref{algoline: mark users unchecked}), which is used to identify good clusters in the current accuracy level. If all users in a cluster are checked, then this cluster is {\it checked} to be an accurate cluster in the current phase. Compute the estimated weight vectors for each cluster (line \ref{algoline: set pivot}), which serve as the pivots to be compared for splitting its containing users. Note that the pivot weight vectors are denoted as $\tilde{\btheta}^j$ instead of $\hat{\btheta}^j$.

At each time $t$ in the $s$-th phase, a user $\bi_{\tau}$ comes to be served with candidate item set $\bD_{\tau}$ (line \ref{algoline: receive user and item set Dt}), where $\tau$ denotes the index of the total time step (line \ref{algoline: compute total time step tau}). 
First obtain the information $(\bS^{\bj}, \bb^{\bj}, \bT^{\bj})$ for the cluster $\bj$ of user $\bi_\tau$ (line \ref{algoline: get cluster index and its associated information}) and then recommend based on these information (line \ref{algoline: recommend item to the user with largest U}). Here $\norm{x}_A = \sqrt{x^\top A x}$ for any positive definite matrix $A$.
After receiving feedback $\by_\tau$, the learner will {\it update} information (Algorithm \ref{alg:update}) and check if a split is possible (Algorithm \ref{alg:split}). 

By the assumptions in \cref{sec:setting}, users in one cluster have same weight vector and same frequency. Thus if a cluster is a good cluster, which only contains users of same underlying cluster, the estimated parameters for containing users will be close to estimated parameters of the cluster. We call a user $i$ is \textit{consistent} with the current cluster $j$ if $\hat{\theta}_i$ is close to $\hat{\theta}^j$ and $\hat{p}_i$ is close to $\hat{p}_{i'}$ for any other user $i'$ of cluster $j$. If a user is inconsistent with the current cluster, the learner will split her out (\cref{alg:split}).

We call two checked clusters \textit{consistent} if their estimated weight vectors and estimated frequencies are close enough. The algorithm will merge two checked clusters if they are consistent (Algorithm \ref{alg:merge}). Here $\hat{p}^j = T^j / (\abs{C^j} \tau)$ is the average frequency of cluster $j$. The condition of clusters to be \textit{checked} is to avoid merging two clusters that are not accurate enough in the current level. The operations of split and merge, together with the conditions, can guarantee that the clusters are good at the end of each phase in the corresponding accuracy level with high probability (the analysis is part of the regret bound proof). 
% The analysis will be provided later.


==> Improved Algorithm on Online Clustering of Bandits/Experiments.tex <==
\section{Experiments}

\begin{figure*}[thb!]
\centering
{\small (1) Synthetic Dataset}\\
\includegraphics[width = 0.24\textwidth]{figs/syna.pdf}
\includegraphics[width = 0.24\textwidth]{figs/synb.pdf}
\includegraphics[width = 0.24\textwidth]{figs/sync.pdf}\\
{\small (2) MovieLens and Yelp Datasets}\\
\includegraphics[width = 0.24\textwidth]{figs/mla.pdf}
\includegraphics[width = 0.24\textwidth]{figs/mlc.pdf}
\includegraphics[width = 0.24\textwidth]{figs/yelpa.pdf}
\includegraphics[width = 0.24\textwidth]{figs/yelpc.pdf}
\caption{
The figures compare \sclub (red) with \club (black), \linucbone (green) and \linucbind (yellow). The first row is for synthetic experiments and the second row is for real datasets, MovieLens and Yelp.
All the experiments are of $n_u=10^3$ users with $d=20, L=20$. We set $m=10$ for (1) synthetic experiments. (1a)(2a)(2c) are of uniform distribution over users, (1b) is of arbitrary distribution over clusters, where the users in the same cluster have the same frequency probabilities, (1c)(2b)(2d) are of arbitrary distribution over users. All results are averaged under $10$ random runs and the errorbars are computed by standard errors, which are standard deviations divided by $\sqrt{10}$.
\vspace{-0.3cm}
}
\label{fig:results}
\end{figure*}

\sclub algorithm is compared with \club \cite{gentile2014online}, \linucbone which uses a single estimated weight vector for all users and \linucbind which uses a separate estimated weight vector for each user on both synthetic and real datasets.

\subsection{Synthetic experiments} 

We consider a setting of $n_u=10^3$ users with $m=10$ clusters where each cluster contains equal number of users. The weight vectors $\theta_1, \ldots, \theta_m$ and item vectors at each round are first randomly drawn in $d-1$ ($d=20$) dimension with each entry a standard Gaussian variable, then normalized, added one more dimension with constant $1$, and divided by $\sqrt{2}$. The transformation is as follows
\begin{equation}
\label{eq:transform x}
x\mapsto \left(\frac{x}{\sqrt{2}\norm{x}},\ \frac{1}{\sqrt{2}}\right)\,. 
\end{equation}
This transformation on both the item vector $x$ and weight vector $\theta$ is to guarantee the mean $\ip{\theta, x}$ lies in $[0,1]$.
The parameters in all algorithms take theoretical values.
The comparisons on theoretical computational complexities of these algorithms is put in
\ifsup
\cref{sec:complexity of implementation}.
\else
supplementary materials.
\fi
The evolution of the regret as a function of time is shown in the first row of \cref{fig:results}
\footnote{The parameters of \club are theoretical values and might be suboptimal. We do not optimize the parameters of any algorithm and just use theoretical values of the parameters in all algorithms including \sclub.}
. The regrets at the end and total running times are given in
\ifsup
\cref{table:regrets} and \cref{table:running time}.
\else
supplementary materials.
\fi
The left figure (a) is under the setting of uniform distribution over all users where each user has a frequency $1/n_u$; middle figure (b) is under the setting of arbitrary distribution over clusters where the users in the same cluster have the same frequency probability; right figure (c) is under the setting of arbitrary distribution over users.

The performance of \sclub improves over \club by $5.94\%$ (\cref{fig:results}(1a)) even in the setting of \club where the frequency distribution over users is uniform. The reason is that \club uses connected components of graphs to represent clusters and if it wants to identify the underlying cluster of a user $i$, it has to delete every bad edge of its neighbors (and neighbors of neighbors, etc.). In comparison, \sclub is much faster, will split a user $i$ out if it finds any inconsistency from her current running cluster, and merge her to any consistent running cluster. The improvement is enlarged to be $13.02\%$ (\cref{fig:results}(1b)) in the setting of \cref{sec:setting} where users in the same cluster have the same frequency probability but users in different clusters might have different frequencies. \sclub is robust in the setting of arbitrary distribution over users where the assumptions in \cref{sec:setting} might fail and can still improve over \club by $14.69\%$ (\cref{fig:results}(1c)).


\subsection{Real datasets} 

We use the $20m$ MovieLens dataset \cite{harper2016movielens} which contains $20$ million ratings for $2.7\times 10^4$ movies by $1.38 \times 10^5$ users and Yelp dataset\footnote{\url{http://www.yelp.com/dataset\_challenge}} 
% \cite{yelp} 
which contains $4.7$ million ratings of $1.57 \times 10^5$ restaurants from $1.18$ million users. The Yelp dataset is more sparse than MovieLens. For each of the two real datasets, we extract $10^3$ items with most ratings and $n_u = 10^3$ users who rate most. Then use the rating matrix to derive feature vectors of $d-1$ ($d=20$) dimension for all users by singular-value decomposition (SVD). The feature vectors are also processed as \eqref{eq:transform x} and the resulting vectors are regarded as the underlying weight vectors of each user. 
% These feature vectors can be visualized in

The performances are shown in \cref{fig:results}(2) where (2a)(2b) are for MovieLens dataset and (2c)(2d) are for Yelp dataset. (2a)(2c) are under the setting of uniform distribution over users and (2b)(2d) are under the setting of arbitrary distribution over users. Since there is no underlying clustering over the users, we do not experiment on the setting of arbitrary distribution over clusters like \cref{fig:results}(1b). The algorithms of \sclub and \club adaptively find finer and finer clustering as more data flows in. The performance of \sclub improves over \club by $5.94\%, 14.84\%, 5.94\%, 16.24\%$ respectively.



==> Improved Algorithm on Online Clustering of Bandits/Introduction.tex <==
\section{Introduction}

The problem of stochastic multi-armed bandit (MAB) \cite{bubeck2012regret,LS18book} has been widely studied in the field of statistics and machine learning, where the learner selects an action each round with the goal of maximizing the cumulative rewards over all rounds (or equivalently minimize the cumulative regret). 
One successful application of MAB algorithms is recommendation systems \cite{aggarwal2016recommender}, such as recommendations of movies, restaurants and news articles. For the setting where new users and items constantly appear where simultaneous exploration and exploitation are naturally needed, bandit algorithms can cope with the ``cold start'' problem and improve itself as time goes on.

To adjust bandit algorithms for large-scale applications, structural assumptions are usually added on actions and reward functions, among which linear structure is one of the most common due to its simplicity and effectiveness. Each item in the stochastic linear bandits \cite{abe1999associative,rusmevichientong2010linearly,dani2008stochastic,abbasi2011improved} is represented by a feature vector whose expected reward is an unknown linear function on the feature vector. In many systems certain side information about users and items are employed as the feature vectors to guarantee recommendation quality \cite{li2010contextual,chu2011contextual}.

Usually user features are not accurate enough or even do not exist to characterize user preferences. When user features exist, these static features are usually combined together with item features to be actions in linear bandit models. This processing might have implacable modeling bias and also neglect the often useful tool of collaborative filtering. One way to utilize the collaborative effect of users is to discover their clustering structure. Clustering methods have been proved to be important in supervised/unsupervised recommendations \cite{linden2003amazon,woo2014cluster}. The works \cite{gentile2014online,li2016collaborative} start to bring these useful techniques to bandit algorithms. These online clustering of bandit algorithms adaptively learn the clustering structure over users based on the collaborative recommendation results to gather information of users' similarity and still keep certain diversity across users.

There are two main challenges in the existing works on online clustering of bandits \cite{gentile2014online,li2016collaborative,korda2016distributed,gentile2017context,li2016art}. (a) The existing works assume users come to be served in a uniform manner. However, as stated by long tail effect and $80/20$ rule, the imbalance between users always exist especially with a large number of low-frequency users. The low-frequency users deteriorate the performance of existing algorithms. (b) The existing works use graphs to represent users, use edges to denote the similarity between users and use connected components to represent clusters. 
As a result, the learner may split two dissimilar users into two clusters only when it cuts every path between these two users. Even when the edge (representing the similarity) between two users are cut, the two users might still need to stay in the same cluster for a long time. Therefore these algorithms are not efficient in identifying the underlying clusters.

To overcome the first problem, we include frequency properties into the criterion of an underlying clustering structure. To overcome the second problem, we split a user out of her current cluster once we find the current cluster contains other users dissimilar to this one. Since the split operation might be a bit radical and premature, we add a new merge operation to reconcile the radical effect of the split operation. Based on these two building operations, complex graph structure can be discarded and replaced by simple set structures where each cluster is represented by a set of users.

This paper makes four major contributions:
\begin{enumerate}
\item We generalize the setting of online clustering of bandits to allow non-uniform frequency distributions over users.

\item We design both split and merge operations on clusters together with set representations of clusters to accelerate the process of identifying underlying clusters.

\item We analyze the regret of our new algorithm to get a regret bound free of the term $1/p_{\min}$, where $p_{\min}$ is the minimal frequency probability among all users and the existing algorithms could not avoid it.

\item We compare our algorithm to the existing algorithms on both synthetic and real datasets. A series of experiments consistently show the advantage of our algorithm over the existing ones.
\end{enumerate}

\subsection{Related work} 

The most related works are a series of studies on online clustering of bandits. \citet{gentile2014online} first establish the setting of online clustering of bandits and first show the effectiveness of using graph structure to represent clustering over users. A follow-up \cite{li2016collaborative} considers the collaborative filtering effects on both users and items but only under the setting of static item pool. They maintain a clustering over items and for each item cluster there is a clustering over all users. Their analysis is only built on a special case that the items form an orthonormal basis in the feature space. Based on \cite{gentile2014online}, \citet{korda2016distributed} design a distributed version of confidence ball algorithms in peer to peer networks with limited communications where the peers in the same cluster solve the same bandit problem. \citet{gentile2017context} present a context-aware clustering bandit algorithm where the clustering structure depends on items, though with a high computational cost. All these works assume the user frequency distribution is uniform and use connected components of graphs to represent clusters. 

Besides these works with new algorithms and theoretical guarantees, there are many progress of applying these online algorithms in real applications. \citet{nguyen2014dynamic} design a variant of clustering of bandit algorithms by performing k-means clustering method \cite{macqueen1967some} on the estimates of user weight vectors with a known number of clusters. 
\citet{christakopoulou2018learning} present a variant of clustering of bandit algorithms based on Thompson sampling and allow recommending a list of items to users.
\citet{kwon2018overlapping} allows the underlying clustering has overlapping.
All these works focus on experimental performance and do not include theoretical guarantees, especially on regret bounds.
\citet{li2018online} study an application of using clustering of bandit algorithms to improve the performance of recommending a list of items under a specific click model, and they provide a regret guarantee.

There is a group of works on stochastic low-rank bandits \cite{katariya2017stochastic,katariya2017bernoulli,kveton2017stochastic}. They assume the reward matrix of users and items are of low-rank and the learner selects a user-item pair each time. The goal of the learner is to find the user-item pair that has the maximum reward. This is different from the setting of online clustering of bandits where there is no control over user appearances and the goal of the learner is to maximize satisfaction of each appearing user.

The works on linear bandits are cornerstones of clustering of bandits, where the latter has different weight vectors and adaptively clusters users. It is first studied by \cite{abe1999associative} and refined by \cite{dani2008stochastic,abbasi2011improved} and many others. \citet{turgay2018multi} present a similar work to make use of collaborative results but they assume the similarity information is known.


% The problem of stochastic multi-armed bandit (MAB) has been widely studied in the field of statistics and machine learning \cite{bubeck2012regret,LS18book}. Classically it is formulated as a system of $K$ arms whose rewards are random samples from unknown but fixed distributions. The learning agent pulls one arm at each time step and the goal is to maximize the cumulative reward in expectation. The measure of performance is often the cumulative regret, defined as the difference in the expected cumulative reward between always pulling the best arm (the arm with the highest expected reward) and the pulling by the learning agent. At a high level, the agent needs to strike the balance between choosing the arm that has exhibited the best performance \textit{so far} (exploitation), and trying other arms that have not been explored enough yet (exploration). A frequentist's technique to deal with this exploitation-vs-exploration trade-off with near optimal regret bound is based on the principle of optimism in face of uncertainty (OFU). More specifically, one computes confidence intervals of each arm's expected reward and uses the upper confidence bounds (UCBs) as criteria for expected rewards \cite{lai1985asymptotically,auer2002finite}. The midpoint of the confidence interval for an arm is the sample mean of the rewards, and the confidence radius (half the length of the interval) shrinks as the arm is played more and more. As the upper confidence bound is the midpoint plus the confidence radius, the UCB criterion deals with the trade-off by simultaneously taking exploration and exploitation into account.
	
% In some applications, the arms or the rewards have their own structures, motivating researchers to explore settings beyond the classical MAB. Recent examples include combinatorial MABs \cite{cesa2012combinatorial,gai2012combinatorial,chen2016combinatorial,combes2015combinatorial}, (stochastic) linear bandits \cite{auer2002using,dani2008stochastic,abbasi2011improved,agrawal2013thompson} and a combination of the two \cite{qin2014contextual}. In combinatorial MABs, the learning agent chooses a \textit{super arm}, which is a \textit{set} of base arms instead of only one arm. Different feedback models can be considered: If the learning agent receives the reward of each individual base arm in the selected super arm, the feedback is called \textit{semi-bandit}; if the learning agent only receives a total reward of the super arm, the feedback is called \textit{bandit}. In linear bandit setting, the learning agent chooses an item represented by a vector $x$ and receives a random reward with mean being the inner product of the vector $x$ with a fixed but unknown weight vector $\theta$. If the reward of the super arm is the sum of the rewards of the base arms, then the setting of combinatorial MAB with bandit feedback can be regarded as a special case of the linear bandits.
	

% In this paper, we study online clustering of bandits to combine online cluster learning with online recommendations. Clustering methods have been proved to be important in offline recommendations \cite{linden2003amazon,woo2014cluster}, and also start to shine in the online setting \cite{gentile2014online,li2016collaborative,korda2016distributed,gentile2017context}. The existing online clustering of bandit algorithms are graph-based, where they represent each user by a node and use connected components to denote clusters. They will check the edge between every pair of users, which might be quite inefficient when the number of users is large.
% % If there are a large number of users, it is not very efficient to compute connected components of the large graph at each round. 
% Also due to the privacy and safety reasons, when a user comes to be served, the learning agent might only have the access to this user's information and some aggregated information among users. Lack of other individual users' information will make existing graph-based methods inapplicable.
% 	% the information of other users, thus the current graph-based clustering methods might not be applicable.
% Moreover, existing works assume that the probabilities of all users coming online are the same, which is unrealistic in practice. A straightforward adaption of existing works to the nonuniform user probability case would lead to undesirable regret bound that has a large term $\frac{1}{p_{\min}}$ (see Theorem \ref{thm:club}), where $p_{\min}$ is the minimum user visit probability.
	
% In this paper, we bring up a set-based method to online clustering of bandits to address the above issues. We prove an upper bound of $\tilde{O}(\sqrt{T})$ for the cumulative regret, where $T$ is the number of total rounds. Moreover, our regret bound is better for the nonuniform user visit probability by removing the dependency on the $\frac{1}{p_{\min}}$ term. Our algorithm only maintains aggregate information on clusters and never store individual user's information, and thus it has the added benefit of privacy consideration. Finally, our experiments demonstrate that our algorithm provides better regret with a shorter running time comparing to the previous solution on clustering of bandits.
		
% The organization of this paper is as follows. Section 2 introduces previous work related to our setting; Section 3 formulates the setting of {\it Online Clustering of Bandits in Large-Scale Recommendations} with some appropriate assumptions; Section 4 gives our set-based algorithm SCLUB and the cumulative regret bound; Section 5 reports experimental results; Section 6 concludes the paper.

% There have been quite a number of papers on linear payoff functions as ours \cite{auer2002using,dani2008stochastic,abbasi2011improved,li2010contextual}. Dani et al. \cite{dani2008stochastic} considers stochastic linear bandit setting and provides two algorithms based on $L^2$-norm and $L^1$-norm estimations. Abbasi-Yadkori et al. \cite{abbasi2011improved} uses a martingale technique to get an improved regret bound. They also prove a high probability constant regret bound for classical MAB as a special case. Agrawal et al. \cite{agrawal2013thompson} considers a similar setting but with Thompson sampling approach. The works of \cite{li2010contextual,chu2011contextual,qin2014contextual} apply linear bandit setting in the application of online recommendations. Our setting also considers a linear payoff but assumes different users might have different weight vectors and explores the clustering structure over users online.

% The work \cite{gentile2014online} first considers the setting of online clustering of linear bandits, where they maintain a graph among users and used connected components to denote user clusters. Korda et al. \cite{korda2016distributed} designs a distributed version of confidence ball algorithms in peer to peer networks. And then a follow-up \cite{li2016collaborative} explores item structures to help cluster users, where they also maintain a clustering over items and constructed a user clustering for each item cluster. Their limitation is that the item set should be static, or only has a small change along the time. A recent work proposed in \cite{gentile2017context} presents a context-aware clustering bandit algorithm, though with a high computational cost. All above works are graph-based and use connected components in graphs to represent clusters. In this paper we employ sets to represent clusters and manage to make it to work in a more general setting where user appearance probabilities might not be the same. 

% The study \cite{kveton2017stochastic} considers a setting of stochastic low-rank bandits where the learning agent selects a user-item pair each time and the objective is to find a user-item pair which has the maximum reward. However our setting has no control over user appearances and the objective is to find maximum item for each user.

==> Improved Algorithm on Online Clustering of Bandits/Results.tex <==
\section{Results}

Recall that $d$ is the feature dimension, $m$ is the (unknown) number of clusters and $n_u$ is the number of users. Let $n^j$ be the (unknown) number of users in cluster $j$ and $p^j$ be the (unknown) frequency for cluster $j$, which is the sum of (unknown) user frequencies in cluster $j$. The following main theorem bounds the cumulative regret of our algorithm \sclub.
\begin{theorem}
\label{thm:main}
Suppose the clustering structure over the users, user frequencies, and items satisfy the assumptions stated in \cref{sec:setting} with gap parameters $\gamma, \gamma_p > 0$ and item regularity parameter $0 < \lambda_x \le 1$. Let $\alpha_{\theta} = 4 R \sqrt{d/\lambda_x}$, $\alpha_p = 2$ and
$\beta = R \sqrt{d \ln(1 + T / d) + 2 \ln(4 m n_u)}$. Then the cumulative regret of the algorithm \sclub after $T$ rounds satisfies
\begin{align} \label{eq:SCLUBregret}
R(T) &\le \sum_{j=1}^m 4 \beta \sqrt{d p^j T \ln(T/d)}  \notag \\
&\quad + O\left( \left(\frac{1}{\gamma_p^2} + \frac{n_u}{\gamma^2 \lambda_x^3}\right) \ln(T) \right)\\
&= O(d\sqrt{m T} \ln(T))\,.
\end{align}
\end{theorem}
\begin{proof}[sketch]
The proof is mainly based on two parts. The first part bounds the exploration rounds to guarantee the clusters partitioned correctly. The second part is to estimate regret bounds for linear bandits after the clusters are partitioned correctly.

By Chernoff-Hoeffding inequality, we prove when
$
\tau \ge O\left(\frac{1}{\gamma_p^2}\ln(T) + \frac{1}{p_i}\ln(T) \right)
$
the distance of $p_i$ and $\hat{p}_i$ is less than $\gamma_p/2$. Then the users with different frequencies will be assigned to different clusters. Thus, the cluster containing user $i$ only contains users with the same frequency probabilities, for all user $i$.

Then by the assumption of item regularity, when
$
\tau \ge O \left(\frac{1}{\gamma_p^2}\ln(T) + \frac{1}{p_i}\ln(T) + \frac{1}{p_i \gamma^2 \lambda_x^3} \ln(T) \right)
$
the estimated weight vectors will be accurate enough for all the users with the frequency probability same as $p_i$. The 2-norm radius for the confidence ellipsoid of the weight vector will be less than $\gamma/2$. Thus the split and merge operations will function correctly for users. Next, we prove that if two clusters containing the users of same frequency probabilities have accurate estimates for weight vectors and frequencies, the combined cluster inherits the accuracies with high probability. Thus, the combination steps can continue until it contains all users of an underlying cluster.

After the cluster $j$ with frequency probability $p^j$ is correctly partitioned, the recommendation is based on the estimates of cluster weight vector. The regret for the second part reduces to linear bandits with $p^j T$ rounds.
\end{proof}


The proof is much different from that of \club \cite{gentile2014online} with the additional frequency probability and merge operation. 
The full proof is put in 
\ifsup
\cref{sec:proof of sclub}.
\else
the supplementary materials.
\fi


% \begin{proof}[Sketch]
% The proof is mainly based on two parts. The first part bounds the exploration rounds to guarantee when the clusters will be partitioned correctly. The second part is to estimate regret bounds of linear bandits for the true clusters.

% By Chernoff-Hoeffding inequality, when
% $
% \tau \ge O\left( \frac{1}{\gamma_p^2} \ln(T) + \frac{1}{p_i}\ln(T) \right)
% $,
% the distance of $p_i$ and $\hat{p}_i$ is less than $\gamma_p / 4$, where $\gamma_p$ is the gap between user frequencies. Then the users with different frequencies will be assigned to different clusters. Thus for any user $i$, the cluster containing user $i$ only contains users with the same frequency probabilities. 

% Then by the assumption of item regularity, when
% $
% \tau \ge O\left( \frac{1}{p_i} \ln(T) + \frac{1}{p_i \lambda_x^2} \ln(T) + \frac{R}{p_i \gamma_{\theta} \lambda_x} \sqrt{\ln(T)} \right)
% $,
% the estimated weight vectors will be accurate enough for all the users with the frequency probability same as $p_i$. The $2$-norm radius for the confidence ellipsoid of the weight vector will be less than $\gamma / 2$, where the $\gamma$ is the gap between user weight vectors. Thus, the condition for the split and merge will function correctly for users. Note that after multiplying the frequency $p_i$ for user $i$, the $p_i$ in the denominator will be cancelled out.

% Next, if two sub-clusters of the true cluster, which means they have the same weight vectors and same user frequencies, have estimates accurate enough, the merged cluster inherits the accuracy properties. Thus, the merge steps will start from two users in the same true cluster, and will continue until the resulting cluster is the true cluster.

% After the true cluster $j$ with frequency probability $p^j$ is correctly formed, the recommendation is based on the estimates of weight vector on the cluster. The regret for this part is reduced to the setting of linear bandits with $p^j T$ rounds for each true cluster $j$.
% \end{proof}

\subsection{Discussions}

First, we compare our regret bound with that of \club. Since \club is designed and proved only for uniform distribution over users, we first generalize the regret bound of \club to the setting of arbitrary distribution over users.
\begin{theorem}
\label{thm:club}
Under the same setting with \sclub, the cumulative regret of the algorithm, \club, after $T$ rounds satisfies
\begin{align*} \label{eq:CLUBregret}
R(T) &\le \sum_{j=1}^m 4 \beta \sqrt{d p^j T \ln(T/d)} + O\left(\frac{1}{p_{\min} \gamma^2 \lambda_x^3} \ln(T) \right)\\
  &= O(d \sqrt{m T} \ln(T))\,.
\end{align*}
\end{theorem}
Note that in the degenerate setting where the distribution $p$ over users is uniform, $p_{\min} = 1 / n_u$ and the regret bound recovers the one in the previous work \cite{gentile2014online}.

In real applications, there might be a lot of infrequent users with frequency close to $0$. Since the algorithm \club initializes with a complete graph or a random connected graph, there would be a lot of infrequent users connecting with frequent users. Infrequent users receive a recommendation once a long time. Thus it takes a long time to differentiate them from frequent users, or to be split into a different cluster (connected component) from frequent users. Then the recommendations for frequent users would be polluted by these infrequent and dissimilar users for a long time. The length of rounds to separate infrequent dissimilar users is proportional to $1/p_{\min}$, the minimal frequency over all users. $p_{\min}$ could be arbitrarily small in real applications, the $\log$ term in regret bound for \club is not satisfactory. Due to an additional care on frequencies, \sclub could get rid of the uncontrollable term $1 / p_{\min}$.

The assumption that users with same weight vectors have same frequencies is based on the intuition that frequent users and infrequent users usually have different preferences. It can be relaxed to that users with same weight vectors have close frequencies. For more general cases, a new structure of nested clusters could help where the infrequent users could use the information of frequent users but not vice versa. We leave this as interesting future work.

Second, our result can be generalized by allowing multiple users each round. In applications the recommender system will update itself every a fixed time slot, and during each time slot, multiple users will be served using the same history information. 
\begin{theorem}
\label{thm:multiple users}
Under the same setting with \sclub, each user appear with frequency $p_i \in [0, 1]$, then the cumulative regret of the algorithm after $T$ rounds satisfies
\begin{align*}
R(T) &\le \sum_{j=1}^m 4 \beta \sqrt{d p^j T \ln(T/d)} \\
&\quad + O\left( \left(\frac{\bar{p}}{\gamma_p^2} + \frac{n_u}{\gamma^2 \lambda_x^3}\right) \ln(T) \right)
\end{align*}
where $\bar{p} = \sum_{i = 1}^{n_u} p_i$ is the sum of all user frequencies.
\end{theorem}
Note this recovers the regret bound in \cref{thm:main} when $\bar{p} = 1$. The regret bound for \club can also be generalized in a similar way.

Third, if the clustering structure is known, the setting would be equivalent to $m$ independent linear bandits, each with the expected number of rounds $p^j T$. Then the regret bound would be $O(d\sum_{j=1}^m\sqrt{p^j T} \ln(T))$ by \cite{abbasi2011improved} which matches the main term of ours \eqref{eq:SCLUBregret}. The upper bound reaches its maximum $O(d\sqrt{m T} \ln(T))$ when $p^1 = \cdots = p^m = 1/m$. Also the regret lower bound in this case is $\Omega(\sum_{j=1}^m \sqrt{d p^j T})$ by \cite{dani2008stochastic} which matches the main term of \eqref{eq:SCLUBregret} up to a term of $\sqrt{d} \ln(T)$.

Fourth, we would like to state the additional benefit of \sclub in privacy protection. To protect user privacy, when a user $i$ comes to be served, the learning agent will have the only access to the information of user $i$ and some aggregate information among users, but does not have the access to other individual users' information. In this sense, lack of other individual users' information will make existing graph-based methods \cite{gentile2014online,li2016collaborative} inapplicable. Our algorithm \sclub only uses information of user $i$ and aggregate information of clusters to split and merge.

Due to space limit, more discussions are put in
\ifsup
\cref{sec:more discussions}.
\else
the supplementary materials.
\fi

% Setting reasonable gap parameters would help to identify a good clustering and improve the recommendation quality. Furthermore, as more data flows in, the parameters can be changed smaller and our algorithm can continue working without the need to restart. By a similar analysis, we could derive an asymptotic regret bound (with parameters in the algorithm changed accordingly). We omit this part and simply assume the gap exists.



% The assumption that there is a true clustering structure over users is not as restrictive as it looks. Our algorithm, as well as other graph-based clustering bandit algorithms, leverages exploration time on the hidden clustering structures to improve the recommendation quality. Furthermore, the assumptions on the gap parameters are further relaxed as more data flows in. Our algorithm explores clustering structures adaptively, as well as other clustering bandit algorithms. It starts with one cluster, then finds finer and finer clustering. The cluster cardinality $m$ is determined by the selected parameters and unavoidable (see the third statement above).

% Last, we discuss other assumptions. We assume the learning agent has no control over user appearances and at each time step, each user is drawn independently with her own frequency probability. If the learning agent has the access to sampling users, the setting is a bit different and should have a better regret bound because the learning agent does not need to wait for collecting enough information. 

% The assumption on items is to guarantee that the confidence ellipsoid for any weight vector will shrink, thus the learning agent is able to distinguish them after collecting enough information. If this assumption is violated, we can specify a barycentric spanner in the item set, as adopted in \cite{dani2008stochastic}. The work \cite{lattimore2017end} also discusses the importance of incorporating a barycentric spanner to achieve efficiency in learning.



==> Improved Algorithm on Online Clustering of Bandits/Setting.tex <==
\section{Model and Problem Definitions}
\label{sec:setting}

In this section, we formulate the setting of ``online clustering of bandits''. There are $n_u$ users, denoted by the set $[n_u] = \{1, \ldots, n_u\}$, with a fixed but {\em unknown} distribution $p = (p_1, \ldots, p_{n_u}) \in \Delta_{n_u}$ over users. Here $\Delta_{n} = \{ x \in [0,1]^n: \sum_{i=1}^n x_i = 1 \}$ denotes the simplex in $\RR^n$. There is also a fixed but {\em unknown} distribution $\rho$ over $\{x \in \RR^d: \norm{x} \le 1\}$, which is the set of feature vectors for all items, and we simply call such a feature vector an item. At each time $t$, a user $\bi_t \in [n_u]$ is randomly drawn from the distribution $p$, and $L$ items are drawn independently from distribution $\rho$ to form a feasible item set $\bD_t$. The learning agent receives the user index $\bi_t$ and the feasible item set $\bD_t$, selects an item $\bx_{t} \in \bD_t$ and recommends it to the user. After the user checks the item $\bx_t$, the learning agent receives a reward $\by_t$. The setting follows the previous work \cite{gentile2014online} but allows non-uniform distribution over users.
	
Let $\cH_t = \{\bi_1, \bx_1, \by_1, \ldots, \bi_{t-1}, \bx_{t-1}, \by_{t-1}, \bi_t\}$ be all the information after receiving the user index in time $t$. Then the action $\bx_{t}$ is $\cH_{t}$-adaptive. Henceforth, we will write $\EEt{\cdot}$ for $\EE{\cdot \mid \cH_{t}}$ for the sake of notational convenience, use the boldface symbols to denote random variables, and denote $[n]$ to be the set $\{1,\ldots,n\}$.
	
For any time $t$, given a fixed user $i$ at time $t$ and a fixed item $x \in \bD_t$ selected for user $i$, we define the random reward of item $x$ for user $i$ to be $\by_t(i,x) = \theta_i^\top x + \bvarepsilon_{i, t, x}$, where (a) $\theta_{i}$ is a fixed but {\em unknown} weight vector in $\RR^{d \times 1}$ with $\norm{\theta_{i}} \le 1$, independently of other items and other user behaviors; and (b) $\bvarepsilon_{i,t,x}$ is an $\cH_t$-conditional random noise with zero mean and $R$-sub-Gaussian tail, i.e. $\EE{\exp(\nu\bvarepsilon_{i,t,x})} \le \exp(R^2 \nu^2/2)$ for every $\nu \in \RR$. Then the mean reward is $\EE{\by_t(i,x)} = \theta_i^\top x$. At time $t$, the learning agent recommends $\bx_t$ to user $\bi_t$ and receives reward $\by_t(\bi_t, \bx_t)$, which satisfies
\begin{align*}
    \EEt{\by_t(\bi_t, \bx_t) \mid \bi_t, \bx_t} = \EE{\by_t(\bi_t, \bx_t) \mid \cH_t, \bi_t, \bx_t} = \theta_{\bi_t}^{\top} \bx_t\,.
\end{align*}

Suppose there are $m$ (unknown) different weight vectors in the set $\{\theta_i :  i \in [n_u]\}$. An underlying clustering exists over the users according to the weight vectors, where the users with the same weight vector form a cluster. The goal is to learn the underlying clustering to help the recommendation process. We make the following assumptions on the weight vectors $\{\theta_i : i \in [n_u]\}$, the distribution $p$ over users, and the distribution $\rho$ on items.

% (see Section Discussions)
	
\paragraph{Gap between weight vectors.} For any two different weight vectors $\theta_{i_1} \neq \theta_{i_2}$, there is a (fixed but unknown) gap $\gamma$ between them: $\norm{\theta_{i_1} - \theta_{i_2}} \ge \gamma > 0$.

\paragraph{Item regularity.} For item distribution $\rho$, $\mathbb{E}_{\bx \sim \rho}[\bx \bx^{\top}]$ is full rank with minimal eigenvalue $\lambda_x > 0$. Also at all time $t$, for any fixed unit vector $\theta \in \RR^d$, $(\theta^{\top} \bx)^2$ has sub-Gaussian tail with variance parameter $\sigma^2 \le \lambda_x^2 /(8 \log(4 L))$. We assume a lower bound for $\lambda_x$ is known.
	
\paragraph{Gap between user frequencies.} Users with same weight vectors will have same frequencies: $\theta_{i_1} = \theta_{i_2}$ implies that $p_{i_1} = p_{i_2}$. Also for any two different user frequency probabilities $p_{i_1} \neq p_{i_2}$, there is a (fixed but unknown) gap $\gamma_p$ between them: $\abs{p_{i_1} - p_{i_2}} \ge \gamma_p > 0$.

All the assumptions except the last one follow the previous work \cite{gentile2014online}. The first part of last assumption could be relaxed. Discussions are provided in a later section.
% \footnote{Interested readers are recommended to refer to the \cite{gentile2014online,li2016collaborative,korda2016distributed,li2018online} for the discussions on the setting and other assumptions.}.
	
The optimal item for user $\bi_t$ in round $t$ is $x_{\bi_t, \bD_t}^\ast = \argmax_{x \in \bD_t} \theta_{\bi_t}^\top x$. Then the expected regret for user $\bi_t$ in time $t$ is $\bR_t = \theta_{\bi_t}^\top x_{\bi_t, \bD_t}^\ast - \theta_{\bi_t}^\top \bx_{t}$. The goal of the learning agent is to minimize the expected cumulative regret 
\begin{align*}
    R(T) = \EE{\sum_{t=1}^{T} \bR_t} = \EE{\sum_{t=1}^{T} \left( \theta_{\bi_t}^\top x_{\bi_t, \bD_t}^\ast - \theta_{\bi_t}^\top \bx_{t} \right) }\,,
\end{align*}
where the expectation is taken over the randomness of users $\bi_1, \ldots, \bi_T$, the randomness of the item sets $\bD_1, \ldots, \bD_T$ and the possible randomness in selected items $\bx_1, \ldots, \bx_T$.
	

==> Improved Algorithm on Online Clustering of Bandits/technical_lemmas.tex <==
\section{Technical Lemmas}

\begin{lemma}[Hoeffding's Inequality \cite{hoeffding1963probability}]
\label{lem:additive chernoff bound}
Let $X_1, \ldots, X_n$ be independent random variable with common support $[0, 1]$. Let $\bar{X} = \frac{1}{n} \sum_{i=1}^n X_i$ and $\EE{\bar{X}} = \mu$. Then for all $a \ge 0$,
\begin{align*}
&\PP{\bar{X} - \mu \ge a} \le  \exp(- 2 n a^2),\quad \PP{\bar{X} - \mu \le -a} \le  \exp(- 2 n a^2)\,.
\end{align*}
\end{lemma}

% \begin{lemma}[Bernstein's Inequality]
% 	\label{lem:Bernstein's inequality}
% 	Let $X_1, \ldots, X_n$ be independent random variable with range $[0, 1]$ and $\sum_{t=1}^n Var[X_t \mid X_{t-1}, \ldots, X_1] = \sigma^2$. Let $S_n = \sum_{i=1}^n X_i$. Then for all $a \ge 0$,
% 	\begin{align*}
% 		\PP\left[S_n \ge \EE[S_n] + a\right] \le  \exp\left(-\frac{a^2/2}{\sigma^2 + a/3}\right)\,.
% 	\end{align*}
% \end{lemma}

\begin{lemma} \label{lem:T-for-ratio-less-than-gamma}
\begin{align*}
\frac{R \sqrt{d \ln(1 + \frac{T}{d}) + 2\ln\frac{1}{\delta_2} } + \sqrt{A(\delta_1)}}{\sqrt{T\lambda_x/8}} < \frac{\gamma}{4}  
\end{align*}
is satisfied when
\begin{align*}
T > \frac{8}{\gamma^2 \lambda_x}\max\left\{A(\delta_1), \quad 4R^2d\log\frac{32R^2}{\gamma^2 \lambda_x}, \quad 4R^2\ln\frac{1}{\delta_2} \right\}\,.
\end{align*}
\end{lemma}
\begin{proof}
To prove this, it is enough to prove $\frac{\sqrt{A(\delta_1)}}{\sqrt{T\lambda_x/8}} \le \frac{\gamma}{8}$ and $\frac{R \sqrt{d \ln(1 + \frac{T}{d}) + 2\ln\frac{1}{\delta_2} }}{\sqrt{T\lambda_x/8}} < \frac{\gamma}{8}$.

The first condition is equivalent to $T \ge \frac{8 A(\delta_1)}{\gamma^2 \lambda_x}$. 

The second condition can be derived by $(a) \frac{d\ln(1+T/d)}{T\lambda_x} < \frac{\gamma^2}{16 R^2}$ and $(b)\frac{2\ln\frac{1}{\delta_2}}{T\lambda_x} < \frac{\gamma^2}{16 R^2}$. (a) is satisfied when $T > \frac{32R^2d}{\gamma^2 \lambda_x}\log\frac{32R^2}{\gamma^2 \lambda_x}$ by \cite[Lemma 9]{li2019online}. (b) is equivalent to $T > \frac{32R^2}{\gamma^2 \lambda_x}\ln\frac{1}{\delta_2}$.

Thus summarizing the three conditions for $T$ to finish the proof.
\end{proof}

\begin{lemma} \label{lem:selfNorm}
Let $M_n = M + \sum_{t=1}^n \sum_{k=1}^{K_t} x_{t,k} x_{t,k}^{\top}$, where $M \in \RR^{d \times d}$ is a strictly positive definite matrix and $x_{t,k} \in \RR^d$ is a $d$-dimensional column vector. If $\sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}^2 \leq 1$, then
\begin{equation}
\sum_{t=1}^n \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}^2 \leq 2\log\frac{\det(M_n)}{\det(M)}\,.
\end{equation}
Furthermore, if $\norm{x_{t,k}}_2 \leq L, K_t \le A, \EE{K_t} = K, M = \lambda I, \lambda \geq A L^2, \forall t,k$, then
\begin{equation}
\label{eq:selfNormSum}
\sum_{t=1}^n \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}} \leq \sqrt{2dnK \log\left(1 + \frac{n A L^2}{\lambda d}\right)}.
\end{equation}
\end{lemma}
\begin{proof}
\begin{align*}
&\det(M_n)= \det(M_{n-1}) \det\left(I + M_{n-1}^{-1/2} \left(\sum_{k=1}^{K_n}x_{n,k} x_{n,k}^{\top} \right) M_{n-1}^{-1/2} \right)\\
\overset{(a)}{\ge}& \det(M_{n-1}) \left(1 + \sum_{k=1}^{K_n} \norm{x_{t,k}}_{M_{n-1}^{-1}}^2 \right) \ge \det(M) \prod_{t=1}^n \left(1 + \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}^2 \right),
\end{align*}
where (a) is by Lemma A.3 of \cite{li2016contextual}. Then
\begin{align*}
\sum_{t=1}^n \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}^2 \overset{(b)}{\le} \sum_{t=1}^n 2 \log\left(1 + \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}^2 \right) \le 2\log\frac{\det(M_n)}{\det(M)}\,,
\end{align*}
in which (b) is due to $2\log(1+u) \geq u$ for $u\in[0,1]$.

If $\norm{x_{t,k}}_2 \leq L, K_t \le A, \EE{K_t} = K, M = \lambda I, \lambda \geq A L^2, \forall t,k$, then
\begin{align*}
&\EE{\sum_{t=1}^n \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}} \le \left( \EE{\sum_{t=1}^n \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}} }^2 \right)^{1/2} \le \left( \EE{\sum_{t=1}^n K_t \sum_{k=1}^{K_t} \norm{x_{t,k}}_{M_{t-1}^{-1}}^2} \right)^{1/2} \\
\le &\left( \EE{\sum_{t=1}^n K_t \cdot 2 \log\frac{\det(M_n)}{\det(\lambda I)}} \right)^{1/2} \le \sqrt{2dnK \log\left(1 + \frac{n A L^2}{\lambda d}\right)}.
\end{align*}
\end{proof}

